Weight Re-Mapping for Variational Quantum Algorithms

Inspired by the remarkable success of artificial neural networks across a broad spectrum of AI tasks, variational quantum circuits (VQCs) have recently seen an upsurge in quantum machine learning applications. The promising outcomes shown by VQCs, such as improved generalization and reduced parameter training requirements, are attributed to the robust algorithmic capabilities of quantum computing. However, the current gradient-based training approaches for VQCs do not adequately accommodate the fact that trainable parameters (or weights) are typically used as angles in rotational gates. To address this, we extend the concept of weight re-mapping for VQCs, as introduced by K\"olle et al. (2023). This approach unambiguously maps the weights to an interval of length $2\pi$, mirroring data rescaling techniques in conventional machine learning that have proven to be highly beneficial in numerous scenarios. In our study, we employ seven distinct weight re-mapping functions to assess their impact on eight classification datasets, using variational classifiers as a representative example. Our results indicate that weight re-mapping can enhance the convergence speed of the VQC. We assess the efficacy of various re-mapping functions across all datasets and measure their influence on the VQC's average performance. Our findings indicate that weight re-mapping not only consistently accelerates the convergence of VQCs, regardless of the specific re-mapping function employed, but also significantly increases accuracy in certain cases.

==> contents/2_preliminaries.tex <==
%\section{\uppercase{Preliminaries}}
%Variational quantum circuits (VQCs) gained huge popularity in quantum machine learning (QML) over the past years. The idea of VQCs is drawn from artificial neural networks, where massively parameterized function approximators allow unprecedented success in a vast number of tasks in AI. Making use of the richer algorithmic toolbox available in quantum computing, the introduction of VQC has already shown promising results, e.g., in generalization and the need for less training steps and data. \cite{schuld_introduction_2015,cerezo_variational_2021}
%JS: we miss somthing about the data embeddings here

\section{Variational Quantum Circuits}
Variational Quantum Circuits can be seen as a quantum analog to classical artificial neural networks (ANNs). ANNs use parameterized linear transformations in combination with non-linear activation functions applied to artificial neurons. These parameters - usually called weights and biases - can be trained to increase the ANNs performance qualitatively. Corresponding optimization approaches are predominantly gradient based techniques, which mainly rely on the efficiency of backpropagation. It has been shown in Cybenko's universal approximation theorem, that ANNs with sufficiently many neurons can approximate arbitrary functions with arbitrary precision, showing their vast applicability in many different areas of research.~\cite{Cybenko1989} Contrary to ANNs, where the information processed resides in the activation of neurons, the information in quantum circuits is described by the state of a qubit register $\ket{\psi_i}$, which denotes a normalized vector in a specific Hilbert space $\mathcal{H}$. The application of functions on these qubit registers are formalized by unitary operators $U$, which map an initial state $\ket{\psi_i}$ to a final state $\ket{\psi_f}$ as a linear function $\ket{\psi_i} \mapsto \ket{\psi_f} = U\ket{\psi_i}$. To extract classical information from a quantum system, a so called measurement must be applied. Such measurements yield an eigenvalue of a particular Hermitian operator $O$, which is typically chosen to be the spin Hamiltonian in the $z$-axis. According to the Born rule, the expected value when applying such a measurement operator can be calculated with $\bra{\psi_f}O\ket{\psi_f}$.\\

\noindent Observing that concatenations of unitary operators also resemble a unitary operator yields that the operation described by a VQC is described completely by a single parameterized unitary operator $U(\theta)$. Vice versa, every unitary operator can be decomposed into a set of basic quantum gates, i.e.,  rotational (ROT) and controlled-not (CNOT) gates. In the underlying Hilbert space, these operations represent rotations and reflections, respectively~\cite{nielsen_chuang_2010}. For VQCs, this decomposition notably allows for concentrating the parameters in the rotational gates only, leaving the CNOT gates parameter-free. These ROT gates are fully described by a rotation axis an angle in the Bloch sphere. Mathematically, these observations lead to describing the expected output of a VQC as
\begin{equation}
    \bra{\psi_f(\theta)}O\ket{\psi_f(\theta)}
\end{equation}
In integral part of constructing a quantum function approximator using a VQC is choosing a suitable circuit structure, often called ansatz. By additionally employing an adequate objective function, the parameters are then typically trained using a quantum-classical pipeline, as displayed in Figure~\ref{fig:structure}.

\noindent The standard method to calculate gradients of the parameters $\theta$ in VQCs is the parameter shift rule \cite{schuld_evaluating_2019}. In contrast to the classically employed backpropagation, this technique has a linear time complexity in the number of parameters. This is considerably worse than the backpropagation, which has constant runtime in the number of parameters. However, current research is actively trying to tackle this problem~\cite{abbas2023quantum}.


%The most prominent function approximator used in classical machine learning is the artificial neural network: a combination of parameterized linear transformations and typically non-linear activation functions, applied to neurons. The weights and biases used to parameterize the linear transformations can be updated using gradient based techniques like backpropagation, optimizing the approximation quality. According to Cybenko's universal approximation theorem, this model allows the approximation of arbitrary functions with arbitrary precision.\cite{Cybenko1989}. 

%In a quantum circuit, information is stored in the state of a qubit register $\ket{\psi_i}$, i.e., normalized vectors living in a Hilbert space $\mathcal{H}$. In quantum mechanics, a function mapping the initial state $\ket{\psi_i}$ onto the final state $\ket{\psi_f}$ is expressed by a unitary operator $U$ that maps the inputs onto the outputs as in $\ket{\psi_f} = U \ket{\psi_i}$. In contrast to classical outputs, quantum outputs can only be obtained via so called measurements, which yield an eigenstate corresponding with an expected value of $\bra{\psi_f}O\ket{\psi_f}$, where $O$ is typically chosen to be the spin Hamiltonian in the $z$-axis. %Measuring each qubit individually

%In order to build a quantum function approximator in form of a VQC, one typically decomposes the arbitrary unitary operator $U$ into a set of quantum gates. Analogously to Cybenko's theorem, in the quantum case it can be proved that any unitary operator acting on multiple qubits can always be expressed by the combination of controlled-not (CNOT) and rotational (ROT) gates, which represent reflections or rotations of the vector into the Hilbert space respectively \cite{nielsen_chuang_2010}. While CNOTs are parameter-free gates, each rotation is characterized by the three angles around the axes of the Bloch sphere. These rotation parameters are the weights of the quantum variational circuit. We can thus say that the final state actually depends on the weights $\theta$ of the circuit, and rewrite the output final value as 
%\begin{equation}
%    \bra{\psi_f(\theta)}O\ket{\psi_f(\theta)}
%\end{equation}
%Starting from this theoretical basis, a function approximator can be obtained once a suitable circuit structure, also called ansatz, has been chosen. Once this is done and an objective function has been chosen, the rotation weights can be trained in a quantum-classical pipeline, as shown in Figure \ref{fig:structure}, completely analogously to what is done with a neural network.

%Similar to a classical neural network, where the gradient is calculated using backpropagation, we can differentiate the circuit with respect to the parameters $\theta$ in a similar way using the parameter shift rule \cite{schuld_evaluating_2019}. It has to be noted however, that this approach has linear time complexity in the number of parameters and every gradient calculation has to be executed on a quantum computer. This is significantly worse than the constant time complexity regarding the number of parameters, needed in backpropagation.

%It can in fact be proved that

% \begin{align*}
%    \frac{\partial \bra{\psi_f(\theta)}O\ket{\psi_f(\theta)}}{\partial \theta} =\\
%    \frac{1}{2} ( \bra{\psi_f(\theta + \pi/2)}O\ket{\psi_f(\theta + \pi/2)} \\
%    - \bra{\psi_f(\theta - \pi/2)}O\ket{\psi_f(\theta - \pi/2)}) 
%\end{align*}


% Which means that in order to compute the gradient we just have to run the same circuit again twice with the parameters shifted of $\pm \pi/2$

% Similar to classical machine learning, variational quantum circuits (VQC) contain weights within their structure that need to be adjusted for a correct function approximation of the whole circuit. A VQC is a hybrid between a classical circuit and a quantum one, where a quantum circuit is measured against a known set of training and label data and its weights adjusted via a classical computer. \cite{cerezo_variational_2021} The functional structure of the quantum circuit is fixed and its structure largely based on the experience of the researcher, whereas continuous rotation matrices act as elements corresponding to weights in classical machine learning. Both the structure (sometimes called ansatz) of the circuit and the best structure of the cost function in the feedback loop are areas of active development \cite{zhang_fast_2022, hellstern_analysis_2021,lubash_variational_2020} but outside of the scope of this work. 

%\subsection{Data embeddings}
%JS: ich würde hier viel weniger mathemtisch generell bleiben, es is doch alles super straight forward wenn man schreibt dass Schaltkreise in Rotationen und CNOTs zerlegt werden können. Alle Parameter landen in den Rotationen und die erlauben nunmal logischerweise Parameter von 0 bis 2pi. Klar das man seine Daten da anpassen sollte, motivation ist da dann natürlich auch dass wir bei so nem preprocessing auch klassisch schon Erfolge sehen. 
%Already in classical machine learning, transforming raw ("uncurated") data with simple transformations is a basic step in most machine learning applications \cite{ezukwoke_data_}. Typically it entails rescaling the data for a mean of zero and adjusting the variance for a consistent performance of the applied machine learning algorithm.\todo{check and confirm} In the classical case, both the data and the weights within the function approximator live in the same domain $\mathbb{R}$. Compare this with quantum computing, where the individual data input on a single qubit is in $SU(2)$ and the weights on each axially restricted rotation matrix on $S^1$ or $SU(2)$ for universal rotation matrices. This change of domain requires a transformation function from classical data space to an embedding on the quantum computer inputs. 
